Coherent Probabilistic Aggregate Queries on Long-horizon Forecasts

Long range forecasts are the starting point of many decision support systems that need to draw inference from high-level aggregate patterns on forecasted values. State of the art time-series forecasting methods are either subject to concept drift on long-horizon forecasts, or fail to accurately predict coherent and accurate high-level aggregates. In this work, we present a novel probabilistic forecasting method that produces forecasts that are coherent in terms of base level and predicted aggregate statistics. We achieve the coherency between predicted base-level and aggregate statistics using a novel inference method based on KL-divergence that can be solved efficiently in closed form. We show that our method improves forecast performance across both base level and unseen aggregates post inference on real datasets ranging three diverse domains. (\href{https://github.com/pratham16cse/AggForecaster}{Project URL})

==> aggregate_queries.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{|l|l|l|r|r|}
        \hline
        Dataset & aggregate & $K$ & No-\Our & \Our \\ \hline
        Solar & Avg. & 2 & 14.5825 & 13.276 \\  % With OPT-SUM
            &   & 3 & 14.1208 & 12.7678 \\
            &   & 6  & 13.1424 & 11.8111 \\
            &   & 12  & 12.5047 & 11.1406 \\
            &   & 24  & 11.2528 & 10.6176 \\ \cline{2-5}
            & Slope. & 2 & 14.8924 & 13.6739 \\
            &   & 3  & 14.5493 & 13.4153 \\
            &   & 6  & 17.1474 & 15.9805 \\
            &   & 12  & 15.9239 & 16.2313 \\
            &   & 24  & 0.6569 & 0.6568 \\ \cline{2-5}
            & Diff. & 2 & 8.3059 & 8.0629 \\
            &   & 3  & 10.7434 & 10.7803 \\
            &   & 6  & 17.5359 & 16.9646 \\
            &   & 12  & 23.9637 & 22.0572 \\
            &   & 24  & 24.8199 & 17.4107 \\ \hline

		ETT (R96) & Avg. & 2 &   0.9385 & 0.9299 \\ 
			&  & 3 &   0.9337 & 0.9251 \\
			&  & 6 &   0.9228 & 0.9143 \\
			&  & 12 &   0.9022 & 0.8948 \\
			&  & 24 &   0.8684 & 0.8616 \\ \cline{2-5}
			& Slope & 2 &   0.9403 & 0.9319 \\
			&  & 3 &   0.9368 & 0.9286 \\
			&  & 6 &   0.9262 & 0.9187 \\
			&  & 12 &   0.9182 & 0.9093 \\
			&  & 24 &   0.8908 & 0.8824 \\ \cline{2-5}
			& Diff & 2 &   0.2177 & 0.2173 \\
			&  & 3 &   0.2463 & 0.246 \\
			&  & 6 &   0.305 & 0.3022 \\
			&  & 12 &   0.4121 & 0.3979 \\
			&  & 24 &   0.4999 & 0.4956 \\ \hline
			
		Taxi & Avg. & 2  &  2.6619 & 2.6318 \\
			&  & 3  &  2.5318 & 2.5054 \\
			&  & 6  &  2.3488 & 2.3119 \\
			&  & 12  &  2.0914 & 2.0373 \\
			&  & 24  &  1.8929 & 1.8133 \\ \cline{2-5}
			& Slope & 2  &  2.9686 & 2.9338 \\
			&  & 3  &  2.9843 & 2.9323 \\
			&  & 6  &  3.039 & 2.9569 \\
			&  & 12  &  3.3582 & 3.2776 \\
			&  & 24  &  3.1166 & 3.2985 \\ \cline{2-5}
			& Diff & 2  &  3.1483 & 3.1654 \\
			&  & 3  &  3.0067 & 2.9896 \\
			&  & 6  &  2.6976 & 2.7904 \\
			&  & 12  &  2.8839 & 2.8828 \\
			&  & 24  &  2.3555 & 2.5307 \\ \hline
			
ETT(R192) & sum  & 1  & 3.064800 & 3.069400 \\ 

 & & 3  & 2.791300 & 2.727000 \\ 

 & & 4  & 2.723900 & 2.611100 \\ 

 & & 6  & 2.601200 & 2.450400 \\ 

 & & 12  & 2.341300 & 2.203100 \\ 

 & & 24  & 2.068800 & 1.952200 \\ 

& slope  & 1  & 3.064800 & 3.069400 \\ 

 & & 3  & 2.911000 & 2.887100 \\ 

 & & 4  & 2.864000 & 2.842100 \\ 

 & & 6  & 2.802000 & 2.776800 \\ 

 & & 12  & 2.624200 & 2.567000 \\ 

 & & 24  & 2.259300 & 2.103100 \\ 

& diff  & 1  &  nan &  nan \\ 

 & & 3  & 1.323000 & 1.453500 \\ 

 & & 4  & 1.388600 & 1.656000 \\ 

 & & 6  & 1.310600 & 1.545000 \\ 

 & & 12  & 1.384100 & 1.333800 \\ 

 & & 24  & 1.468500 & 1.432100 \\ 

    \end{tabular}
    \caption{Results on Aggregate Queries with SUM aggregate model}
    \label{tab:aggregate_queries}
\end{table}


==> figures/agg_results_table.tex <==
\begin{table*}
\centering
\begin{tabular}{|l|l|l|r|r|r|r|r|r|r|}
\hline
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Agg} & \multirow{2}{*}{Model} & \multicolumn{7}{c|}{K} \\ \cline{4-10}
 & & & 2 & 3 & 4 & 6 & 8 & 12 & 24 \\ \hline

\etth & \sumagg & \TransformerNAR & 1.87 & 1.902 & 1.921 & 1.938 & 1.93 & 1.924 & 1.891 \\
& & \sharq & 1.672 & 1.632 & 1.628 & 1.637 & 1.67 & 1.569 & 1.514 \\
& & \Our & 1.623 & 1.603 & 1.645 & 1.675 & 1.691 & 1.711 & 1.729 \\
\cline{2-10}

& \slopeagg & \TransformerNAR & 0.476 & 0.311 & 0.256 & 0.192 & 0.196 & 0.137 & 0.066 \\
& & \Our & 0.87 & 0.519 & 0.334 & 0.181 & 0.171 & 0.114 & 0.057 \\
\cline{2-10}

& \diffagg & \TransformerNAR & 0.238 & 0.595 & 0.27 & 0.292 & 0.388 & 0.458 & 0.504 \\
& & \Our & 0.435 & 0.581 & 0.365 & 0.335 & 0.356 & 0.386 & 0.414 \\
\hline


\ett & \sumagg & \TransformerNAR & 1.307 & 1.339 & 1.358 & 1.379 & 1.389 & 1.391 & 1.379 \\
& & \Our & 1.213 & 1.142 & 1.198 & 1.195 & 1.22 & 1.239 & 1.264 \\
\cline{2-10}

& \slopeagg & \TransformerNAR & 0.315 & 0.178 & 0.132 & 0.089 & 0.074 & 0.064 & 0.048 \\
& & \Our & 0.588 & 0.401 & 0.226 & 0.086 & 0.091 & 0.061 & 0.04 \\
\cline{2-10}

& \diffagg & \TransformerNAR & 0.157 & 0.401 & 0.143 & 0.144 & 0.156 & 0.204 & 0.29 \\
& & \Our & 0.294 & 0.421 & 0.248 & 0.221 & 0.206 & 0.211 & 0.247 \\
\hline


\electricity & \sumagg & \TransformerNAR & 54.15 & 53.79 & 53.56 & 52.79 & 52.3 & 50.81 & 48.42 \\
& & \Our & 50.81 & 50.64 & 50.59 & 50.07 & 49.67 & 48.43 & 46.28 \\
\cline{2-10}

& \slopeagg & \TransformerNAR & 13.99 & 11.42 & 8.959 & 7.487 & 6.248 & 5.654 & 2.233 \\
& & \Our & 12.67 & 10.33 & 8.26 & 6.911 & 5.764 & 5.185 & 2.137 \\
\cline{2-10}

& \diffagg & \TransformerNAR & 6.996 & 19.33 & 9.503 & 11.57 & 13.23 & 18.37 & 16.13 \\
& & \Our & 6.334 & 17.63 & 8.797 & 10.52 & 12.22 & 16.84 & 15.44 \\
\hline


\solar & \sumagg & \TransformerNAR & 13.62 & 13.63 & 13.25 & 12.99 & 12.95 & 12.78 & 12.43 \\
& & \Our & 13.04 & 13.1 & 12.8 & 12.58 & 12.61 & 12.46 & 12.24 \\
\cline{2-10}

& \slopeagg & \TransformerNAR & 6.135 & 5.529 & 4.864 & 4.389 & 3.018 & 4.104 & 0.393 \\
& & \Our & 5.749 & 5.173 & 4.519 & 4.086 & 2.85 & 3.982 & 0.38 \\
\cline{2-10}

& \diffagg & \TransformerNAR & 3.067 & 5.884 & 5.025 & 7.053 & 5.977 & 12.59 & 5.618 \\
& & \Our & 2.874 & 5.534 & 4.678 & 6.557 & 5.587 & 12.26 & 5.376 \\
\hline

\end{tabular}
\end{table*}

% \caption{CRPS of \Our\ and baseline \TransformerNAR\ model on four datasets and three aggregates for different values of window size $K$.}
% \label{fig:aggregate_numbers_table}


% \begin{table*}[]
% \begin{tabular}{lllllllllll}
% \etth & \sumagg   & \TransformerAR  & 1.756 & 1.73  & 1.712 & 1.708 & 1.729 & 1.737 & 1.732 & 1.187 \\
%       &           & \TransformerNAR & 1.566 & 1.597 & 1.625 & 1.664 & 1.697 & 1.712 & 1.657 & 1.313 \\
%       &           & \Our            & 1.514 & 1.546 & 1.575 & 1.616 & 1.669 & 1.702 & 1.649 & 1.255 \\
%       & \slopeagg & \TransformerAR  & 1.571 & 0.847 & 0.588 & 0.341 & 0.137 & 0.061 & 0.038 & 0.027 \\
%       &           & \TransformerNAR & 1.003 & 0.532 & 0.364 & 0.225 & 0.122 & 0.058 & 0.038 & 0.017 \\
%       &           & \Our            & 0.983 & 0.515 & 0.345 & 0.211 & 0.105 & 0.055 & 0.037 & 0.018 \\
%       & \diffagg  & \TransformerAR  & 1.571 & 2.488 & 2.572 & 3.512 & 5.57  & 10    & 18.35 & 196   \\
%       &           & \TransformerNAR & 1.003 & 1.815 & 1.599 & 2.186 & 4.92  & 10.42 & 17.34 & 125   \\
%       &           & \Our            & 0.983 & 1.744 & 1.534 & 2.071 & 4.243 & 9.057 & 17.53 & 132 
% \end{tabular}
% %\caption{Aggregate numbers}
% \label{tabl:aggregate_results}
% \end{table*}

==> figures/main_table.tex <==
\begin{table}%[b!]
\begin{tabular}{|l|l|r|r|r|}
\hline
Dataset & Model & CRPS & MAE & MSE \\ \hline
\ett         & \Informer           & 7.01  & 7.01  & 61.67 \\
            & \TransformerAR         & 3.03  & 3.76  & 19.83 \\
            & \TransformerNAR       & 1.24  & 1.57  & 4.03  \\
            & \Our & \textbf{1.10}  & \textbf{1.55}  & \textbf{3.87}  \\ \hline
\solar       & Informer           & 41.01 & 41.01 & 2810 \\
            & \TransformerAR         & 21.13 & 22.34 & 1683 \\
            & \TransformerNAR       & 13.85 & 14.98 & \textbf{899} \\
            & \Our & \textbf{13.09} & \textbf{14.95} & 906 \\ \hline
\etth   & Informer           & 4.80  & 4.80  & 34.75 \\
            & \TransformerAR         & 1.96  & 2.53  & 10.02 \\
            & \TransformerNAR       & 1.79  & 2.22  & 7.45  \\
            & \Our & \textbf{1.60}  & \textbf{2.19}  & \textbf{7.24}  \\ \hline
\electricity & Informer           & 172.3 & 172.3 & 44689  \\
            & \TransformerAR         & 140.7  & 146.4 & 34702  \\
            & \TransformerNAR       & 54.1 & 56.6 & 6475 \\
            & \Our & \textbf{50.2} & \textbf{55.1} & \textbf{6136} \\ \hline
\end{tabular}
\caption{Comparison of \Our with three baseline models -- (i) \Informer, (ii) \TransformerAR, and (iii) \TransformerNAR using evaluation metrics CRPS, MAE, and MSE. On CRPS and MSE, \Our\ performs better than all the baselines whereas on MAE, \Our\ performs better than baselines in three out of four cases.}
\label{tab:main_table}
\end{table}
%\todo{Informer numbers look too high..Put same number of decimal positions for all numbers.}

==> figures/singleKvsmultK.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{|l|l|r|r|}
\hline
Dataset      & Model           & K      & CRPS   \\ \hline
\ett         & \TransformerNAR & 1       & 1.133  \\ \cline{2-4}
             & \Our            & 4,6,12 & \textbf{1.099}  \\
             &                 & 4      & 1.103  \\
             &                 & 6      & 1.117  \\
             &                 & 12     & 1.122  \\ \hline \hline
\solar       & \TransformerNAR &  1      & 10.242 \\ \cline{2-4}
             & \Our            & 2,6,12 & 10.208 \\
             &                 & 2      & 10.332 \\
             &                 & 6      & 10.225 \\
             &                 & 12     & \textbf{10.094} \\ \hline \hline
\etth        & \TransformerNAR &   1     & 1.547  \\ \cline{2-4}
             & \Our            & 2,6    & \textbf{1.498}  \\
             &                 & 2      & 1.502  \\
             &                 & 6      & 1.524  \\ \hline \hline
\electricity & \TransformerNAR & 1       & 41.527 \\ \cline{2-4}
             & \Our            & 2,6,12 & \textbf{39.937} \\
             &                 & 2      & 40.356 \\
             &                 & 6      & 40.792 \\
             &                 & 12     & 40.738 \\ \hline \hline
\end{tabular}
\caption{Effect of performing inference using single $K$ value versus multiple $K$ values. In all datasets except \solar, using multiple $K$ values yields better forecasts than using single $K$ value.}
\label{tab:ksensitivity}
\end{table}
%\todo{boldface best numbers in all tables}
